Distributed Conditional Cooperation Model Predictive Control of Interconnected Microgrids

In this paper, we propose a model predictive control based operation strategy that allows for power exchange between interconnected microgrids. Particularly, the approach ensures that each microgrid benefits from power exchange with others. This is realised by including a condition which is based on the islanded operation cost. The overall model predictive control problem is posed as a mixed-integer quadratically-constrained program and solved using a distributed algorithm that iteratively updates continuous and integer variables. For this algorithm, termination, feasibility and computational properties are discussed. The performance and the computational benefits of the proposed strategy are highlighted in an illustrative case study.

==> figures/NewNodeCommands.tex <==

\newcommand{\tower}{\begin{tikzpicture}[scale = \scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
         limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] 
				(0,0)
       rectangle (24,24);
   \draw (-1,0) arc (180:360:1cm and 0.5cm);
    \draw (-1,0) arc (180:0:1cm and 0.5cm);
    \draw (-2,-3) arc (180:360:2cm and 1cm);
    %\draw[dashed] (-2,-3) arc (180:10:2cm and 1cm);
    \draw(-2,-3)  -- (-1,0);
    \draw(2,-3)   -- (1,0);
    \shade[left color=blue!5!white,right color=blue!60!white,opacity=0.3] (-1,0) arc (180:360:1cm and 0.5cm) -- (2,-3) arc (360:180:2cm and 1cm) -- cycle;
    \shade[left color=blue!5!white,right color=blue!60!white,opacity=0.3] (0,0) circle (1cm and 0.5cm);
\end{tikzpicture}
}

\newcommand{\GraphTristateFC}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      %\path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (9,12) -- (15,6);
      \path[draw,fill,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth,color=black!50!white] (18,4) rectangle (15,20);
      \path[draw,fill,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth,color=black!80!white] (13,4) rectangle (11,20);
      \path[draw,fill,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth,color=black!50!white] (9,4) rectangle (6,20);
\end{tikzpicture}}

\newcommand{\GraphTristateTF}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (4,12);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (20,12) -- (24,12);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (15,12) circle (5);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (9,12) circle (5);
\end{tikzpicture}}

\newcommand{\GraphTristatePCC}{\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (0,0)
        rectangle (24,24);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (0,12) -- (9,12) -- (15,6);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line width=\lnwidth] (15,12) -- (24,12);
\end{tikzpicture}}

\newcommand{\GraphTristateR}{
%	\renewcommand{\linewidthR}m}
\begin{tikzpicture}[scale = \scaleSymbols, >=latex, color=black]
        \path[] (315.0000,52.3622-1) rectangle (335.0000,72.3622-1);
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=\lnwidth] (324.0306,59.8874) .. controls (321.9302,58.2551) and
          (319.7014,56.9114) .. (317.2333,55.6929) .. controls (319.8093,57.9660) and
          (324.1469,60.6035) .. (324.0306,59.8874) -- cycle;
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=\lnwidth] (325.5865,60.4167) .. controls (328.0392,59.6017) and
          (330.4240,58.6404) .. (332.7667,57.0558) .. controls (329.8032,57.9971) and
          (326.8503,59.6115) .. (325.5865,60.4167) -- cycle;
        \path[draw,fill,line join=round,line cap=round,miter limit=4.00,line
          width=\lnwidth] (324.8607,61.1176) .. controls (324.6795,63.5961) and
          (324.6662,66.1651) .. (325.3315,69.0315) .. controls (325.5549,66.1044) and
          (325.1090,62.6873) .. (324.8607,61.1176) -- cycle;
        \path[cm={{0.20207,0.0904,-0.09626,0.21517,(296.36236,26.26027)}},draw,fill,line
          join=round,line cap=round,miter limit=4.00,line width=\lnwidth]
          (186.0000,84.3622) .. controls (186.0000,86.6957) and (183.5376,88.5874) ..
          (180.5000,88.5874) .. controls (177.4624,88.5874) and (175.0000,86.6957) ..
          (175.0000,84.3622) .. controls (175.0000,82.0287) and (177.4624,80.1370) ..
          (180.5000,80.1370) .. controls (183.5376,80.1370) and (186.0000,82.0287) ..
          (186.0000,84.3622) -- cycle;
\end{tikzpicture}
}

%===================

\newcommand{\GraphTristateS}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (265.0000,52.3622)
          rectangle (285.0000,72.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (269.0000,61.3622) -- (281.0000,61.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (275.0000,55.3622) -- (275.0000,61.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (272.0000,63.3622) -- (278.0000,63.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (275.0000,63.3622) -- (275.0000,69.3622);
\end{tikzpicture}
}


\newcommand{\GraphTristateL}{
\begin{tikzpicture}[scale = -\scaleSymbols*20/24, >=latex, color=black]
      \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (231.3607,117.8948)
        rectangle (255.3607,141.8948);
      \path[draw,line join=miter,line cap=butt,miter limit=4.00,line
        width=\lnwidth, <-] (243.3607,137.3622) -- (243.3607,124.4274);
\end{tikzpicture}
}

% %===================

\newcommand{\GraphTristateT}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (495.0000,52.3622-.5)
          rectangle (515.0000,72.3622-.5);
        \path[cm={{0.38462,0.0,0.0,0.83333,(380.9615,-59.27301)}},draw, line
          join=round,line cap=round,miter limit=4.00,line width=\lnwidth, color = black]
          (342.0000,145.3622) .. controls (342.0000,150.3328) and (333.2695,154.3622) ..
          (322.5000,154.3622) .. controls (311.7305,154.3622) and (303.0000,150.3328) ..
          (303.0000,145.3622) .. controls (303.0000,140.3916) and (311.7305,136.3622) ..
          (322.5000,136.3622) .. controls (333.2695,136.3622) and (342.0000,140.3916) ..
          (342.0000,145.3622) -- cycle;
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth, color = black]
          (505.0000,54.3622) -- (505.0000,69.3622);
\end{tikzpicture}
}


% %===================

\newcommand{\GraphTristateP}{
\begin{tikzpicture}[scale = -\scaleSymbols, >=latex, color=black]
        \path[line join=miter,line cap=round,miter
          limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (495.0000,52.3622)
          rectangle node {N} (515.0000,72.3622) ;
\end{tikzpicture}
}

% %===================

\newcommand{\GraphTristatePV}{
\begin{tikzpicture}[scale =  -\scaleSymbols, >=latex, color=black]
%=== PV ===
  \begin{scope}[cm={{1.33333,0.0,0.0,1.33333,(-219.66665,-77.45405)}}]
    \path[line join=miter,line cap=round,miter
      limit=4.00,line width=\lnwidth,rounded corners=0.0000cm] (371.0000,157.3622)
      rectangle (386.0000,172.3622);
    \begin{scope}[cm={{0.75,0.0,0.0,0.75,(108.84792,54.02778)}}]
      \path[cm={{0.45455,0.21485,-0.21652,0.51139,(295.25671,66.03768)}},draw,fill,line
        join=round,line cap=round,miter limit=4.00,line width=\lnwidth]
        (186.0000,84.3622) .. controls (186.0000,86.6957) and (183.5376,88.5874) ..
        (180.5000,88.5874) .. controls (177.4624,88.5874) and (175.0000,86.6957) ..
        (175.0000,84.3622) .. controls (175.0000,82.0287) and (177.4624,80.1370) ..
        (180.5000,80.1370) .. controls (183.5376,80.1370) and (186.0000,82.0287) ..
        (186.0000,84.3622) -- cycle;
      \begin{scope}[shift={(-0.46388,0.41703)}]
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (362.2097,144.9631) -- (368.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,151.3622) -- (356.4103,149.0251);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (363.3146,147.2675) -- (368.0000,147.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,143.3622) -- (356.1804,145.6575);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (368.0000,155.3622) -- (362.5254,149.6350);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (358.2954,144.1423) -- (356.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (360.0000,155.3622) -- (359.9369,151.0555);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,155.3622) -- (357.0000,150.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,147.3622) -- (356.2119,147.4569);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (352.0000,139.3622) -- (357.1274,144.7105);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (359.8422,144.3002) -- (360.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (361.3258,144.2370) -- (364.0000,139.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (356.0000,155.3622) -- (358.2954,150.8977);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (362.6832,145.9732) -- (368.0000,142.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (363.2514,148.3092) -- (368.0000,149.3622);
        \path[draw,line join=miter,line cap=butt,line width=\lnwidth]
          (364.6693,154.2802) -- (361.4307,150.5189);
      \end{scope}
    \end{scope}
  \end{scope}
\end{tikzpicture}
} 

==> figures/cigreBenchmarkNodeVIII.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = ../paper.tex

\newcommand{\lnwidth}{.7pt}
\newcommand{\lngrid}{0.100pt}

\newcommand{\wInPlot}[2]{\ensuremath{w_{\mathrm{#1},#2}}}
\newcommand{\wDPlot}[1]{\wInPlot{d}{#1}}
\newcommand{\wRPlot}[1]{\wInPlot{r}{#1}}

\newcommand{\xSPlot}[1]{\ensuremath{x_{#1}}}
\newcommand{\pInPlot}[2]{\ensuremath{p_{\mathrm{#1},#2}}}
\newcommand{\pSPlot}[1]{\pInPlot{s}{#1}}
\newcommand{\pTPlot}[1]{\pInPlot{t}{#1}}
\newcommand{\pRPlot}[1]{\pInPlot{r}{#1}}
\newcommand{\pGPlot}[1]{\pInPlot{g}{#1}}

\newcommand{\uInPlot}[2]{\ensuremath{u_{\mathrm{#1},#2}}}
\newcommand{\uSPlot}[1]{\uInPlot{s}{#1}}
\newcommand{\uTPlot}[1]{\uInPlot{t}{#1}}
\newcommand{\uRPlot}[1]{\uInPlot{r}{#1}}

\newcommand{\scaleSymbols}{0.03}
\input{./figures/NewNodeCommands.tex}

\tikzstyle{grid} = [>=latex, line width=\lnwidth, color=black, font=\footnotesize]

\tikzset{midArrow/.style={
		grid,
		draw,%
		decoration={%
			markings,%
			mark=at position 0.5 with \arrow{stealth},%
		},%
		postaction=decorate}}%
\tikzset{endArrow/.style={
		grid,
		draw,%
		decoration={%
			markings,%
			mark=at position 0.8 with \arrow{stealth},%
		},%
		postaction=decorate}}%
\tikzset{invS/.style={rectangle, draw=black, inner sep=0.1pt, line width=\lnwidth, node distance = 25}}
\tikzset{plotNode/.style={rectangle, fill = none, draw = none, inner sep=0.1pt, line width=\lnwidth}}
\tikzset{scaleNode/.style={scale=1}}


\begin{tikzpicture}[xscale = 0.5, yscale = 0.5]

%% Node 1
\draw[grid, -] (2.7*-1.75 - 0.2, 3*0.6) to coordinate (p1grid) (2.7*-1.75+0.2, 3*0.6);

\path[endArrow] (p1grid) -- node[right, yshift = 1, scaleNode]{\textcolor{colorGrid}{\pGPlot{i}}} (2.7*-1.75, 2.7)
	coordinate[xshift = 0] (p1c)
	coordinate[xshift = 70] (p1t)
	coordinate[xshift = -70] (p1b);

%% Node 1
\node[invS, above of = p1t, node distance = 22] (p1storage) {\GraphTristateS};
\node[at = (p1storage.west), xshift = 1, left, scaleNode, grid] {\textcolor{colorStorage}{\xSPlot{i}}};

\node[invS, above of = p1c, node distance = 22] (p1res) {\GraphTristateR};
\node[at = (p1res.west), xshift = 1, left, scaleNode, grid] {\textcolor{colorDemand}{\wRPlot{i}}};

\node[invS, above of = p1b, node distance = 22] (p1thermal) {\GraphTristateT};


\coordinate[above of = p1thermal, node distance = 17] (u1thermal);
\coordinate[above of = p1res, node distance = 17] (u1res);
\coordinate[above of = p1storage, node distance = 17] (u1storage);

\draw[grid, >=stealth, ->] (u1thermal) node[right, yshift=-3]{\uTPlot{i}} -- (p1thermal);
\draw[grid, >=stealth, ->] (u1res) node[right, yshift=-3]{\uRPlot{i}} -- (p1res);
\draw[grid, >=stealth, ->] (u1storage) node[right, yshift=-3]{\uSPlot{i}} -- (p1storage);


\draw[grid, -] (p1t)++(0.2, 0) -- (p1b) -- ++(-0.2, 0);
\draw[midArrow] (p1thermal) -- node[right, scaleNode]{\textcolor{colorThermal}{\pTPlot{i}}} (p1b);
\draw[midArrow] (p1res) -- node[right, scaleNode]{\textcolor{colorRes}{\pRPlot{i}}} (p1c);
\draw[midArrow] (p1storage) -- node[right, scaleNode]{\textcolor{colorStorage}{\pSPlot{i}}} (p1t);

\draw[grid, ->] (p1t) -- ++(0, -0.8) node[left, yshift = 2] {\tiny Load}
	node[right, yshift = 1, scaleNode] {\textcolor{colorDemand}{\wDPlot{i}}};

\node[at = (p1res.east), xshift = -1, right]{\tiny RES};
\node[at = (p1storage.east), xshift = -1, right]{\tiny Storage};
\node[at = (p1thermal.east), xshift = -1, right]{\tiny Thermal};
\node[at = (p1grid.west), yshift = 3, left]{\tiny \parbox{1.4cm}{\flushright Point of common\\[-1pt] coupling}};

\end{tikzpicture}%


==> figures/powerUnits.tex <==
%\newcommand{\plotPowerAndEnergy}[3]{
%	\begin{axis}[%
%		resultsPlot Power,
%		smooth, stack plots=y, stack negative=separate, area style, enlarge x limits=false,
%		xshift = #2,
%		yshift = #3,
%		title = {#1},
%		]
%		\addplot [linestyleStoragePower stacked] table [x=time, y=pS, col sep=comma] {#1} \closedcycle;
%		\addplot [linestyleGrid stacked] table [x=time, y=pG, col sep=comma] {#1} \closedcycle;
%		\addplot [linestyleRes stacked] table [x=time, y=pR, col sep=comma] {#1} \closedcycle;
%		\addplot [linestyleThermal stacked] table [x=time, y=pT, col sep=comma] {#1} \closedcycle;
%		\addplot [linestyleDemand stacked] table [x=time, y=pD, col sep=comma] {#1} \closedcycle;
%%		\addplot [linestyleMaximumRes] table [x=time, y=wR, col sep=comma] {#1};
%		
%	\end{axis}
%	
%	\begin{axis}[%
%		resultsPlot Energy,
%		smooth,
%		xshift = #2,
%		yshift = #3 - 1.7cm,
%		]
%		\addplot [linestyleStorageEnergy] table [x=time, y=x, col sep=comma] {#1};
%		
%	\end{axis}
%	
%	}


\begin{tikzpicture}[font=\scriptsize]

%\plotPowerAndEnergy{figures/simulationMgI.csv}{0cm}{0cm}
%\plotPowerAndEnergy{figures/simulationMgII.csv}{9cm}{0cm}
%\plotPowerAndEnergy{figures/simulationMgIII.csv}{0cm}{-5.9cm}
%\plotPowerAndEnergy{figures/simulationMgIV.csv}{9cm}{-5.9cm}


\end{tikzpicture}%

